Bit-Level Discrete Diffusion with Markov Probabilistic Models: An Improved Framework with Sharp Convergence Bounds under Minimal Assumptions

This paper introduces Discrete Markov Probabilistic Models (DMPMs), a novel discrete diffusion algorithm for discrete data generation. The algorithm operates in discrete bit space, where the noising process is a continuous-time Markov chain that flips labels uniformly at random. The time-reversal process, like the forward noise process, is a jump process with its intensity governed by a discrete analogue of the classical score function. Crucially, this intensity is proven to be the conditional expectation of a function of the forward process, underlining theoretical alignment with score-based generative models. We establish convergence bounds for the algorithm under minimal assumptions, ensuring robustness and efficiency, which we demonstrate through experiments on low-dimensional Bernoulli-distributed datasets and high-dimensional binary MNIST data. The results highlight competitive performance in generating discrete structures compared to the state-of-the-art. This work bridges theoretical foundations and practical applications, advancing the development of effective and theoretically grounded discrete generative modeling.

==> draft.tex <==
% \textbf{Embedding discrete structure in the continuous space. }
% To preserve the benefits of continuous nature, \citet{dieleman2022continuous,chen2022analog} embedded the discrete structure into the Euclidean space while \citet{richemond2022categorical} embedded it into the simplex, then kept using the forward continuous diffusion models. Specifically, \citet{dieleman2022continuous} proposed a continuous diffusion for categorical data, which has some advantages over autoregressive models, such as the ability to perform arbitrary infilling and a flexible sampling procedure. However, it is still not universally used due to the complexity of the training objectives and the lack of a theoretical guarantee. 

% \textbf{Designing the flow processes over the discrete state space. }
% \citet{campbell2022continuous} provided the first complete continuous time framework for denoising diffusion models of discrete data, which used CTMCs to formulate the forward noising process and associated time reversal dynamic. Despite the same idea, this paper has a much more complicated formulation than ours since the CTMCs they used did not have an explicit interpretation. They also used a corrector to bring the distribution of samples closer to the desired marginal, which produced more training cost in practice. In summary, this paper is a good starting point and opens the door to extending the comprehensive results on diffusion models to the discrete structure, and its computational point of view is already provided by \citet{gat2024discrete}. However, it is not widely used due to complex expressions and costly practice training.  

% \textbf{Generator Matching. }Another recent approach to handle discrete data is generative modeling with arbitrary Markov processes using generator matching, introduced by \citet{holderrieth2024generator}. Specifically, \citet{holderrieth2024generator} constructed an appropriate Markov process that transforms a simple distribution into the desired data distribution via the generator, which can be estimated efficiently using a Neural Network. This model can be used for various state spaces, especially for discrete settings. Despite its general application, the generator matching model is still not widely used as it requires a lot of regularity assumptions, the objective is complex, and there is a lack of convergence guarantee.

% \textbf{Masked diffusion models. }One remarkable model to step towards the complex formulations is the "masked" diffusion, a discrete diffusion process first introduced by \citet{austin2021structured}. Recently, \citet{shi2024simplified} established several properties for this model and built a simpler expression of the training objective, which can be rewritten as a signal-to-noise ratio and hide some useful features. However, the theoretical guarantee is still missing and this model is costly to train in practice due to the ratio. 










% \textbf{DMPMs. }Our paper is a step towards closing these gaps. As we have an explicit description of the forward Markov process, we can express the score function as a conditional expectation and avoid signal-to-noise ratio costly training as in \cite{shi2024simplified}. Precisely, we not only provide a simple and low-cost training objective, but also establish the theoretical guarantee for our models in practice.  
